Adaptive Massively Parallel Algorithms for Cut Problems

We study the Weighted Min Cut problem in the Adaptive Massively Parallel Computation (AMPC) model. In 2019, Behnezhad et al. [3] introduced the AMPC model as an extension of the Massively Parallel Computation (MPC) model. In the past decade, research on highly scalable algorithms has had significant impact on many massive systems. The MPC model, introduced in 2010 by Karloff et al. [16], which is an abstraction of famous practical frameworks such as MapReduce, Hadoop, Flume, and Spark, has been at the forefront of this research. While great strides have been taken to create highly efficient MPC algorithms for a range of problems, recent progress has been limited by the 1-vs-2 Cycle Conjecture [20], which postulates that the simple problem of distinguishing between one and two cycles requires $\Omega(\log n)$ MPC rounds. In the AMPC model, each machine has adaptive read access to a distributed hash table even when communication is restricted (i.e., in the middle of a round). While remaining practical [4], this gives algorithms the power to bypass limitations like the 1-vs-2 Cycle Conjecture. We give the first sublogarithmic AMPC algorithm, requiring $O(\log\log n)$ rounds, for $(2+\epsilon)$-approximate weighted Min Cut. Our algorithm is inspired by the divide and conquer approach of Ghaffari and Nowicki [11], which solves the $(2+\epsilon)$-approximate weighted Min Cut problem in $O(\log n\log\log n)$ rounds of MPC using the classic result of Karger and Stein [15]. Our work is fully-scalable in the sense that the local memory of each machine is $O(n^\epsilon)$ for any constant $0 < \epsilon < 1$. There are no $o(\log n)$-round MPC algorithms for Min Cut in this memory regime assuming the 1-vs-2 Cycle Conjecture holds. The exponential speedup in AMPC is the result of decoupling the different layers of the divide and conquer algorithm and solving all layers in $O(1)$ rounds.

==> archive/archive.tex <==

\iffalse
Designing algorithms which are sublinear in space is crucial when the input data does not fit in the memory of available systems. 
In recent years, with the abundance of data and the increasing demand for large scale data processing, the size of datasets easily surpasses that of the typical machine's memory. 
Examples of the problem domains vary from social network graphs to DNA sequences, and efficiently analyzing such datasets has great economic and social impact.
However, to address any problem subject to this restriction efficiently, we need alternative models of computation as the traditional RAM model is no longer feasible in practice. 
One approach to overcome this obstacle is to utilize a large pool of typical machines which have a substantially smaller amount of memory comparing to the input size.
This simple idea is the key ingredient behind the modern distributed processing frameworks such as MapReduce, Hadoop, and Spark that are widely deployed across the industry at very large scales.
The \emph{Massively Parallel computation} ($\MPC$) model is proposed by Karloff et al.~\cite{karloff2010a}, and enhanced in subsequent works~\cite{andoni2014parallel, beame2017communication, goodrich2011sorting}, to provide a theoretical foundation for algorithms implemented on such frameworks.
Nonetheless, it is now considered a standard model for parallel/distributed computation, which gives us a better understanding of how well algorithms are parallelized. 

\fi

\iffalse
\hamed{begin alternative}

During the last decade, the \emph{Massively Parallel computation} (MPC) model attracted a considerable amount of attention. The MPC model was originally proposed to provide a theoretical foundation to algorithms implemented on modern large scale data processing frameworks such as MapReduce, Hadoop, and Spark. 
Nonetheless, it is now considered a standard model for parallel/distributed computation, which gives us a better understanding of how well algorithms are parallelized. 
The key idea behind this model, and also aforementioned frameworks, is to use many machines to compensate for the shortage of space in individual machines. In this model, the data is distributed among a set of machines each with a sublinear memory, and the process is consisted of several rounds. In each round, machines perform an arbitrary amount of computation on their local data independently. At the end of each round, machines can communicate with each other


\hamed{end alternative}

\fi


==> src/abstract-old.tex <==
In the past decade, research on highly scalable algorithms has had significant impact on many massive systems. 
Massively Parallel Computation (MPC), a popular theoretical model with applications in frameworks like MapReduce, Hadoop, Flume, and Spark, has been at the forefront of this research. 
%While great strides have been taken to create highly efficient MPC algorithms for a range of problems, recent progress has been limited by hardness and conjectures like the 1-vs-2 Cycle Conjecture, which postulates that the simple problem of distinguishing between one and two cycles requires $O(\log n)$ MPC rounds.
To combat this, we study Behnezhad et al.'s Adaptive MPC (AMPC), which adds parallel in-round read access to a distributed hash table throughout MPC computation. 
%While remaining practical, this gives algorithms the power to bypass limitations like the 1-vs-2 Cycle Conjecture. 
%We further leverage the power of AMPC by initiating the study of AMPC algorithms for cut problems on graphs, thus allowing us to come up with sublogarithmic algorithms that may not be possible in MPC.


==> src/conclusion.tex <==

\section{Conclusion}

\hamed{AMPC vs PRAM, corollaries, Move[d] to conclusion, beating work-optimal PRAM result though AMPC, converting from AMPC shaves a log, complete 3-way comparison}

\begin{observation}\label{obs:reductions}
Consider an $O(T)$-round $\AMPC$ algorithm with $\machines$ machines each local memory $O(\local)$ for a constant $0 < \epsilon < 1$ where its total running time is $O(\running)$. Then, there is an $O(\running+T\machines\local)$-work $\EREW$ $\PRAM$ algorithm with depth $\D$ that solves the same problem the $\AMPC$ algorithm solves, where $\D$ is the maximum between equivalent $\PRAM$ algorithms that simulate the local computations of every machine in every round.
\end{observation}

\begin{figure}
    \centering
    \input{figs/reductions}
    \caption{The reductions between three parallel models $\PRAM$, $\MPC$, and $\AMPC$ according to~\cite{karloff2010a},~\cite{behnezhad2019massively}, and Observation~\ref{obs:reductions}.}
    \label{fig:reductions}
\end{figure}

\hamed{Adaptivity gap (need to be defined in our results or intro or ampc section), hardness intuition, cite Xiaourui}

==> src/lowdepth-old.tex <==

\section{Generalized Low Depth Tree Decompositions in AMPC}\label{sec:low-depth}

In order to efficiently compute the singleton cuts in parallel, we first need to compute an efficient decomposition of the MST. The low depth tree decomposition Ghaffari and Nowicki~\cite{ghaffari2020massively} introduce is a very specific decomposition with $i$ levels such that at each level, the tree is split into two trees who share a root and no other vertices and are at least $1/3$ the size of the original graph. Unfortunately, it is unclear how to calculate this precise decomposition efficiently in AMPC. To work around this, we introduce a more generalized version of the low depth tree decomposition, show that it can be computed in AMPC, and later show that we can leverage this to obtain our \mc{} algorithm.

\begin{definition}\label{def:lowdepth}
A \textbf{generalized low depth tree decomposition} $D_T$ of some tree $T$ is a labeling of vertices with levels $\ell(v)\in[h]$ for decomposition height $h\in O(\log^2n)$ such that for each level $i$, the connected components of $T^i = \{v\in T: \ell(v) \geq i\}$ have exactly one vertex labeled $i$ each.
\end{definition}

To see what this means, consider the first level. We start by removing all vertices at the first level, which leaves a forest. For each tree in the forest, we must then have exactly one vertex in the second level. We then remove the second level vertices, and are left with an even more refined forest (notice this strategy splits a tree into at least two components, however there may be more). This process continues until the final, isolated vertices are labeled with the final level. Notice that we are guaranteed that at any level $i$, each connected component has exactly one level $i+1$ vertex that it will remove.

It is not that hard to see that Ghaffari and Nowicki's low depth tree decomposition is a specific example of generalized tree decomposition with depth $O(\log n)$. They put a single vertex in the first level and then simply recurse on the two trees in the remaining forest. Note they require additional properties of this decomposition to obtain their result, specifically that each new component has size at least $\frac13$ of the original component, but we will see later that these are not necessary for finding the singleton cuts.

Like Ghaffari and Nowicki in MPC, we prove this can be computed efficiently in, instead, AMPC.

\begin{lemma}\label{lem:treedecomp}
Computing a generalized low depth tree decomposition of an $n$-vertex tree can be done in $O(1/\epsilon)$ AMPC rounds with $O(n^\epsilon)$ memory per machine and $O(n\log^2 n)$ total memory.
\end{lemma}

The rest of this section is dedicated to proving Lemma~\ref{lem:treedecomp}. The formal and complete algorithm is shown in Algorithm~\ref{alg:lowdepthdecomp} and further details and definitions can be found later in this section. At a high level, our algorithm proceeds as follows:
\begin{enumerate}
\item Root the tree and orient the edges [line~\ref{lin:root}].
\item Contract heavy paths in a \textit{heavy-light decomposition} of $T$ into \textit{meta vertices} to construct a \textit{meta tree}, $T_M$ [lines~\ref{lin:heavylightstart} to~\ref{lin:heavylightend}].
\item For each meta vertex, create a \textit{binarized path}, a binary tree whose leaves are the vertices in the heavy path, in order. Expanding meta vertices in this manner yields our \textit{expanded meta tree} [lines~\ref{lin:expandvertsstart} to~\ref{lin:expandvertsend}].
\item Label each vertex with their depth in the expanded meta tree. For all new vertices (i.e., vertices created in step 3) $v$, label $v$ with the depth of the highest vertex $u$ in the same meta node such that $v$ is the leftmost leaf descending from the rightmost child of $u$ in the binarized path of the meta node [lines~\ref{lin:labelvertsstart} to~\ref{lin:labelvertsend}].
\end{enumerate}

Each of these steps correspond to the following subsections. For instance, step 1 corresponds to Section~\ref{sec:low-depth}.1. All relevant terminology related to these steps are additionally found in the corresponding subsections. Lemma~\ref{lem:treedecomp} is proved at the end of the final subsection.

\begin{algorithm}[ht]
\SetAlgoLined
\KwData{A tree $T = (V(T), E(T))$.}
\KwResult{A mapping $\ell:V(T)\to \mathbb{N}$ of tree vertices to levels.}
 Initialize $\ell:V(T)\to \mathbb{N}$\;
 Root and orient $T$\;\label{lin:root}
 Let $T_H = (V(T), \{e\in E(T): e\text{ is heavy}\}$\;\label{lin:heavylightstart}
 Let $\mathcal{P}$ be the connected components of $T_H$\;
 Let $T_M = (\mathcal{P}, \{(P_1,P_2): P_1,P_2\in\mathcal{P}, \exists (u_1,u_2)\in V(P_1)\times V(P_2) \text{ such that } (u_1,u_2) \in E(T)\})$\;\label{lin:heavylightend}
 \For{$v\in T_M$ of heavy path $P_v$ in parallel} {
    Let $\mathcal{O}:V(T_M)\to \mathcal{N}$ be the pre-order numbering of $P_v$\;\label{lin:expandvertsstart}
    Let $V(T_v)$ be a vertex set of size $2|P_v|-1$ with associated indices $1,\ldots,2|P_v|-1$ and $P_v$ assigned to the leaves\;
    For each $u\in V(T_v)$ assign it a parent $p(u)$, the vertex with index $\lfloor u/2\rfloor$\;\label{lin:bintreestart}
    Let $T_v = (V(T_v), \{(u,p(u)):u\in V(T_v)\})$\;\label{lin:bintreeend}
    For each $w\in P_v$, let $\phi$ map $w$ to the vertex in $V(T_v)$ indexed by $|P_v| + \mathcal{O}(w) - 1$\marina{unsure about this}\;\label{lin:mapleaves}
    For each internal node $u\in T_V$, let $d_u$ be the leftmost leaf descendant of the right child of $u$\;\label{lin:expandvertsend}
    For each $u\in T_v$, let $\ell(u)$ be its depth in $T_v$ plus 1\;\label{lin:labelvertsstart}
    For each $u\in P_v$, overwrite $\ell(u) \gets \min_{u'\in T_v: d_{u'}=\phi(u)} d_{T_v}(u')$\;\label{lin:relabel}
    \If{$v$ is not the root of $T_M$}{
        Let $p\in T$ be meta vertex in $T_M$ containing the parent (in $T$) of the first node in the pre-order numbering of $P_v$\;\label{lin:findparent}
        For each $u\in T_v$, add the depth of $p$ in $T_M$ to $\ell(u)$\; \label{lin:broadcast}
    }\label{lin:labelvertsend}
  }
  \KwRet{$\ell$ limited to the original vertices in $T$}\;
 \caption{\textsf{LowDepthDecomp} \\(Computing a generalized low depth tree decomposition of an input tree in AMPC)}
\label{alg:lowdepthdecomp}
\end{algorithm}

\subsection{Rooting the Tree}
Like in Ghaffari and Nowicki, the first thing we need to do in line~\ref{lin:root} of Algorithm~\ref{alg:lowdepthdecomp} is compute an orientation of the edges. Fortunately this, along with rooting the tree, can be done quickly in AMPC by the results of Behnezhad et al.~\cite{behnezhad2019massively} in their Theorem 7.

\begin{lemma}[Behnezhad et al.~\cite{behnezhad2019massively}]\label{lem:orient}
Given a forest $F$ on $n$ vertices, the trees in $F$ can be rooted and edges can be oriented in $O(1/\epsilon)$ AMPC rounds w.h.p. using $O(n^\epsilon)$ local memory and $O(n\log n)$ total space w.h.p.
\end{lemma}

This completes the first step of our algorithm.

\subsection{Meta Tree Construction}\label{sec:metatree}

We also leverage Ghaffari and Nowicki's notion of heavy-light decompositions for our AMPC algorithm, which can be found in lines~\ref{lin:heavylightstart} through~\ref{lin:heavylightend} in Algorithm~\ref{alg:lowdepthdecomp}. This process allows us to quickly decompose the tree into a set of disjoint paths of \textit{heavy edges}, which are defined as follows (note that our definition slightly deviates from Ghaffari and Nowicki~\cite{ghaffari2020massively}, where the heavy edge must extend to the child with the largest subtree without requiring this subtree to be that large, though it is the same as the definition used by Sleator and Tarjan~\cite{sleator1981a}):

\begin{definition}[Sleater and Tarjan~\cite{sleator1981a}]
Given a tree $T$ and a vertex $v\in T$, let $\{u_i\}_{i\in k}$ be the set of children of $v$ where the subtree rooted at $u_1$ is the largest out of all $u_i$. If there is no strictly largest subtree, we arbitrarily choose exactly one of the children with a largest subtree. Then $(u_1,v)$ is a \textbf{heavy edge} and $(u_i,v)$ is a \textbf{light edge} for all $1 < i \leq k$.
\end{definition} 

\begin{figure}
    \centering
    \scalebox{0.77}{\input{figs/heavylight}}
    \caption{The Heavy-Light decomposition of an example tree.}
    \label{fig:heavylight}
\end{figure}

Then the definition of a heavy path follows quite simply.

\begin{definition}[Ghaffari and Nowicki~\cite{ghaffari2020massively}]
Given a tree $T$, a \textbf{heavy path} is a maximal length path consisting only of heavy edges in $T$.
\end{definition}

Ghaffari and Nowicki then make the observation that the number of light edges and heavy paths is highly limited in a tree. This comes from a simple counting argument, where if you consider the path from root $r$ to some vertex $v$, any time you cross a light edge, the size of the current subtree is reduced by at least a factor of 2. This holds even with our different notion of heavy edges since subtrees rooted at children of light edges are still much smaller compared to the subtree rooted at the parent vertex. This bounds the number of light edges between $r$ and $v$, where each pair of light edges are separated by at most one heavy path, and therefore it also bounds the number of heavy paths.

\begin{observation}[Ghaffari and Nowicki~\cite{ghaffari2020massively}]\label{obs:lightheavy}
Consider a tree $T$ oriented towards root $r$. For each vertex $v$, there are only $O(\log n)$ light edges and only $O(\log n)$ heavy paths on the path from $v$ to $r$.
\end{observation}

Using the definition of heavy edge from Sleator and Tarjan~\cite{sleator1981a} instead of from Ghaffari and Nowicki, we get an additional nice property. This is because in our definition, every internal vertex has one descending heavy edge to one child.

\begin{observation}[Sleator and Tarjan~\cite{sleator1981a}]\label{obs:heavypath}
Given a tree $T$ and an internal vertex $v\in T$, $v$ must be on exactly one heavy path. For a leaf $\ell \in T$, $\ell$ must be on at most one heavy path.
\end{observation}

Our first goal is to compute what we call a \textit{meta tree}. This is a decomposition of our tree that will allow us to  effectively handle heavy edges. It is quite analogous to Ghaffari and Nowicki's notion of the heavy-light decomposition, which partitions the tree into heavy and light edges.

\begin{definition}
Given a tree $T$, the \textbf{meta tree} of $T$, denoted $T_M$, comes from contracting all the heavy paths in $T$. We call the vertices of $T$ \textbf{original vertices} and the vertices of $T_M$ \textbf{meta vertices}.
\end{definition}


\begin{figure}
    \centering
    \input{figs/metatree}
    \caption{The \emph{meta-tree} of the same tree from Figure~\ref{fig:heavylight} is demonstrated in this figure.}
    \label{fig:metatree}
\end{figure}

Note that contracting all heavy paths simultaneously is valid because, by Observation~\ref{obs:heavypath}, all heavy paths must be disjoint. Additionally, all internal meta vertices are contracted heavy paths (as opposed to original vertices), again by Observation~\ref{obs:heavypath}. We note that in AMPC, since connectivity is easy, it is additionally quite easy to contract the heavy paths of $T$ into single vertices.

\begin{lemma}\label{lem:heavylight}
Given a tree $T$, the meta tree $T_M$ can be computed, rooted, and oriented in AMPC in $O(1/\epsilon)$ rounds with $O(n^\epsilon)$ memory per machine and $O(n\log^2n)$ total space w.h.p.
\end{lemma}

\begin{proof}
Consider removing light edges from $T$ to create a forest $F$. Run Behnezhad et al.'s AMPC connectivity algorithm~\cite{behnezhad2020parallel}, which satisfies the round and space constraints, to identify the components and contract them. Add the light edges back in to connect contracted nodes. This clearly is $T_M$. Additionally, as before, we run Behnezhad et al.'s~\cite{behnezhad2019massively} AMPC algorithm for orienting the tree. This too falls within the constraints.
\end{proof}

This completes the second step of our decomposition algorithm.

\subsection{Expanding Meta Vertices}

In order to label the vertices, we need a way to handle the heavy paths corresponding to each meta vertex. Let $v\in T_M$ be a meta vertex, and $P_v$ be the heavy path of original vertices in $T$ corresponding to $v$. Note that we have no stronger bound on the length of a heavy path than $O(n)$. Therefore, a recursive partitioning, or labeling of vertices, that has polylogarithmic depth must be able to cleverly divide heavy paths. We can do this with a new data structure.

\begin{definition}
Given some path $P$, a \textbf{binarized path} is an almost complete binary tree $T$ with $|P|$ leaves filled left to right where there is a one-to-one mapping between $P$ and the leaves of $T$ such that the pre-order traversal of $P$ and $T$ limited to its leaves agree.
%, for any $u,u',u''\in P$ that appear in that order (or reversed), if $v$ is the lowest common ancestor of $u$ and $u'$ and $v'$ is the lowest common ancestor of $u$ and $u''$, then $v'$ is an ancestor of $v$ or $v'=v$.
\end{definition}

By ``agree'', we mean that if a vertex $v\in P$ comes before a vertex $u\in P$ in the pre-order traversal of $P$, then it also does in the pre-order traversal of $T$. In other words, if we draw $P$ and the leaves of $T$ where vertices earlier in the pre-order traversals are on the left, then the left-to-right ordering of the vertices is the same. To characterize this tree, we make a quick observation: 

\begin{observation}\label{obs:binarytree}
An almost complete binary tree on $n$ leaves has $2n-1$ vertices, $\lfloor \log_2n\rfloor + 1$ max depth, and every layer is full except the last, which has $2n-2^{\lfloor\log_2 n\rfloor+1}$ vertices.
\end{observation}

Additionally, we can find a relationship between the ancestry of triplets in $P$ based off of the order of the three vertices.

\begin{observation}\label{obs:ancestors}
Given a binarized path $T$ of a path $P$, for any $u,u',u''\in P$ that appear in that order (or reversed), if $v$ is the lowest common ancestor of $u$ and $u'$ and $v'$ is the lowest common ancestor of $u$ and $u''$, then $v'$ is an ancestor of $v$ or $v'=v$.
\end{observation}

\begin{proof}
Consider such a $u,u',u''\in P_v$ that appear in this order (or reversed), and let $v$ and $v'$ be the lowest common ancestors of $u$ and $u'$, and $u$ and $u''$ respectively. Consider traversing from $u$ up the tree from child to parent, and let $p$ be the current vertex. We start with $p=u$ and thus the leaf set of the subtree rooted at $p$ is $L_p = \{u\}$. As we traverse upwards, we add sets of leaves to $L_p$ that are contiguous in $P_v$. Additionally, one vertex is directly adjacent to a vertex from $L_p$ in $P_v$ because $P_v$ was mapped to the leaves of $T_v$ from left to right. Therefore, $L_p$ is a contiguous chunk of $P_v$. Thus, when $u''$ gets added to the subtree (i.e., when $p=v'$) $u'$ must be in $L_p$ too, either because it was added previously or it is being added at the same time. In the former case, $v$ must have happened before $v'$ and thus $v'$ is an ancestor of $v$, and in the latter $v=v'$.
\end{proof}

To create the tree, we do the following for every $v\in T_M$:
\begin{enumerate}
\item Do a pre-order numbering of $P_v$ rooted at the most ancenstral vertex [line~\ref{lin:expandvertsstart}].
\item Create an almost complete binary tree $T_v$ with $|P_v|$ leaves filled left to right [lines~\ref{lin:bintreestart} and~\ref{lin:bintreeend}].
\item Map the vertices in $P_v$ to the leaves of $T_v$ such that the pre-order traversal of $P_v$ and of $T_v$ limited to its leaves agree. For each vertex $u \in P_v$, calculate its ancestors in $T_v$ and add $u$ to the set of leaves in the subtree rooted at those vertices. An internal vertex only needs to keep track of its descendant leaf that is \textit{earliest} in the pre-order traversal on $P_v$ [line~\ref{lin:mapleaves}].
\item Each vertex in $T_v$ who is a right or only child passes its earliest descendant leaf in the pre-order traversal to its parent. This will be the data $d_u$ associated with an internal vertex $u$ [lines~\ref{lin:mapleaves} and~\ref{lin:expandvertsend}].
\end{enumerate}

To formalize the data associated with a vertex:

\begin{definition}
For an internal vertex $u\in T$ for some tree $T$, the \textbf{data $d_u$ associated with $u$} is the leftmost leaf descendant of $u$'s rightmost child.
\end{definition}

Note that the leftmost leaf descendant of a vertex could be the vertex itself if it has no children. Next, it is pretty direct to see that the produced tree is a binarized path.

\begin{observation}\label{obs:binpathcorrect}
The process described above produces a binarized path $T_v$ of $P_v$ for all $v$, where each $u\in T_v$ is labeled with $d_u$.
\end{observation}

We prove that this can be done in the proper constraints.

\begin{lemma}\label{lem:expandverts}
The heavy paths of a tree can be converted into binarized paths with internal nodes $u$ having access to their associated data $d_u$ in $O(1/\epsilon)$ rounds, $O(n^\epsilon)$ local memory, and $O(n\log n)$ total space w.h.p.
\end{lemma}

\begin{proof}
Correctness of the process described in this section is seen in Observation~\ref{obs:binpathcorrect}. Thus we simply need to show how to implement it in AMPC. For the first step, we can directly leverage Behnezhad et al.'s~\cite{behnezhad2019massively} algorithm for pre-order numbering with $O(1/\epsilon)$ AMPC rounds w.h.p. with $O(n^\epsilon)$ local memory and $O(n)$ total space. Next, we must construct a generic almost complete binary tree with $|P_v|$ leaves. Call this tree $T_v$. By Observation~\ref{obs:binarytree}, this has $2|P_v|-1$ vertices, $\lfloor\log_2|P_v|\rfloor+1$ max depth, and each layer is full except the last which has $2|P_v|-2^{\lfloor\log_2|P_v|\rfloor +1}$ vertices. Thus, it is fairly simple to create the set of all vertices in the tree and then connect each vertex to its parent. Each vertex can be given a unique identifier based off its index in the pre-order numbering. For a vertex with index $1<i< 2|P_v|$, its parent's index $j$ can be computed as $j=\lfloor i/2\rfloor$.

Note that the size of the tree is $O(|P_v|)$ but each individual processor computation (i.e., computing the size of the tree, and then having each index connect itself to its parent) can be done in constant space and 2 rounds. Thus in 2 rounds with very low local space, we can create such a tree. Note that we have to construct these trees in parallel, but it is not hard to see that this will only require $O(n\log n)$ total space.

Next, we must map vertices in $P_v$ to the leaves of $T_v$ and additionally label each vertex in $T_v$ with the $P_v$ vertices in its subtree. To do this, consider some $u\in P_v$. Let $i_u$ be the pre-order number of $u$. The index of its corresponding leaf node $u'$ in $T_v$ is $|P_v|+ i_u-1$. Then we can simply traverse the path from $u'$ to the root $r_v$ of $T_v$. Since the depth of $T_v$ is at most $O(\log n)$ and vertices have pointers to their parents, this can be done locally with adaptive access to our distributed hash table. Thus this requires one round, and $u$ can send itself to all of its ancestors in $T_v$. An internal vertex, however, may receive up to $n$ vertices who are leave and descendants, which must be stored in multiple machines. It can then take $O(1/\epsilon)$ rounds to find the earliest leaf descendant in the pre-order decomposition with $O(n^\epsilon)$ local space. After this computation occurs, each internal vertex only requires $O(\log n)$ space for the identifier of its earliest leaf descendant. It then passes this to its parent in one round and forgets about it, thus requiring again only $O(\log n)$ space. Thus the total space again is just $O(n\log n)$.
\end{proof}

\subsection{Labeling Vertices}

Our next goal is to label the vertices with the level they should be split on. Consider, hypothetically, expanding the meta tree $T_M$ such that every heavy path for a meta vertex $v$ is replaced with its binarized path (which is an almost complete binary tree) $T_v$, and the tree continues at the leaves corresponding to the nodes in the heavy path. Note that only some vertices in the hypothetical tree correspond to vertices in the original tree $T$. Specifically, the internal nodes of each component subtree $T_v$ are not vertices in $T$, but the leaves correspond exactly to the vertices in $T$.

\iffalse
\begin{enumerate}
\item For each $v\in T_M$, each vertex $u\in T_v$ finds its depth in $T_v$, indexed by 1 [line~\ref{lin:labelvertsstart}].
\item For each $v\in T_M$, each internal vertex $u\in T_v$ sends its depth to the data $d_u$ which is, as we recall, a leaf in $T_M$. We only need $d_u$ to maintain the smallest depth it was sent. This depth, if ever received, overwrites its own depth [line~\ref{lin:relabel}].
\item For each $v\in T_M$ with parent $p\in T_M$, find the vertex $u$ in $T_p$ that is the parent node of the heavy path (i.e., the parent of the first node in the pre-order decomposition of the path). Broadcast $u$'s depth to all vertices in the heavy path for $v$. If $v$ is the root of $T_M$, the broadcasted depth is 0 [line~\ref{lin:findparent}].
\item For each $v\in T_M$, each vertex $u\in T_v$ adds the broadcasted value to its depth [line~\ref{lin:broadcast}].
\end{enumerate}
\fi

Our vertex labeling will be as follows for each $v\in T_M$ and $u\in T_v$:
\begin{enumerate}
\item Vertex $u$ finds the path $P^u$ from $u$ to the root of $T_M$, assuming the meta vertices are expanded. 
\item Let $u'$ be the highest vertex on $P^u$ and in $T_v$ such that $u$ is the leftmost descendant of the right child of $u$. Note this may be $u$ itself.
\item Label $u$ with the depth of $u'$ in the expanded $T_M$.
\end{enumerate}

We start by making the following observation that there is a one-to-one correspondence between internal vertices and the leaves (minus one leaf) they send their depths to.

\begin{observation}\label{obs:onetoone}
For every $v\in T_{M}$, the leftmost leaf of $T_v$ will receive no depths from internal nodes in $T_M$. Otherwise each internal vertex sends its depth to exactly one leaf, and every leaf except the leftmost receives exactly one depth.
\end{observation}

\begin{proof}
This comes from the simple facts that: (1) a vertex sends its depth to exactly one leaf, (2) each leaf besides one is the leftmost descending leaf of a right child of at least one ancestor, and (3) there is one more leaf than there are internal vertices. (1) is clearly true from our process description and (3) is a property of trees. (2) happens because if we traverse from a leaf to the root and pick the first vertex that comes after traversing an edge to its right child, then this vertex will send its label to that leaf. This must happen at some point on the ancestral path for all leaves except the leftmost leaf of $T_{v}$, which clearly will never receive a depth from an internal vertex.
\end{proof}

Next, we show that the process above leads to a generalized low depth tree decomposition.

\begin{lemma}\label{lem:decompcorrectness}
The process described above finds a generalized low depth tree decomposition of the original tree $T$ of height $h\in O(\log^2 n)$.
\end{lemma}

\begin{proof}
We show this by induction on the level. At the 1st level, we should only partition the graph once. Let $v$ be a vertex labeled 1. The meta vertex containing $v$ must then have depth 1 for this to work, thus it must be in the root meta vertex $u$ of $T_M$. Additionally, $v$ must have been marked with 1 in the third step of this process. This value can only have been passed down by the root of $T_u$. Since the root only passes its depth to a single vertex by Observation~\ref{obs:onetoone}, then that is the only vertex that $v$ can be, and that vertex must be labeled 1. Therefore, there is exactly one vertex at the 1st level.

Consider a connected component $C$ in $T^i=\{v\in T:\ell(v) \geq i\}$ for some level $i\in h$. Let the ``neighborhood'' $N(C)$ be all the vertices in $T\setminus C$ that are adjacent to some vertex in $C$. We will now show that exactly one vertex in $N(C)$ can be in level $i-1$. Assume for contradiction there are two such vertices, $u,v\in N(C)$ with level $i-1$. Let $u'$ and $v'$ be their respective neighbors in $C$. Since $C$ is a connected component, there is a path $P$ from $u'$ to $v'$ containing only vertices in $C$. All of these vertices have level $i$ or higher by the definition of $C$. Tacking on $u$ and $v$ to the start and end of $P$ respectively, there is a path from $u$ to $v$ consisting of vertices $\{u,v\}\cup P$. Since $u$ and $v$ are at level $i-1$, that means every vertex in this path has level $i-1$ or higher. Therefore, $u$ and $v$ must have been in the same connected component $C'$ in the previous level $T^{i-1}$. By induction, that component must have had only one vertex at level $i-1$. This is a contradiction. Alternatively, if $N(C)$ had no $i-1$ level vertex, then $C$ would be a connected component at level $i-1$, which would mean it would have to have exactly one $i-1$ level vertex which is, again, a contradiction. Thus $N(C)$ must have exactly one vertex in level $i-1$.

Let $v\in N(C)$ be the vertex at level $i-1$, and let $u$ be its neighbor in $C$ (note there can only be one since $T$ is a tree). We consider three cases.

Case 1: $u$ is a child of $v$ and they are not on the same heavy path. Let $u_M$ and $v_M$ be the meta vertices in $T_M$ containing $u$ and $v$ respectively. Clearly, $u_M$ is a child of $v_M$ since $u$ is a child of $v$ and $u_M\neq v_M$. Let $b_{u_M}$ be the broadcast value for $T_{u_M}$ in step 3 of the algorithm. Then definitionally $b_{u_M} = \ell(v) = i-1$. Therefore, the only vertex in $T_{u_M}$ that can be at level $i$ is the one whose depth in $T_{u_M}$ indexed by 1 is, which is precisely the single vertex selected by the root of $T_{u_M}$ in step 2. Any other vertex in $C\cap P_{u_M}$ clearly has a larger label. Any other vertex in $C\setminus P_{u_M}$ by connectivity, must be in the heavy path associated with a meta vertex that is a descendant of $u_M$. Since descending through meta vertices in $T_M$ increases the broadcast value by at least 1, then that vertex must have a label that is at least $i-1+2 = i+1$. Thus no other vertices in $C$ can have label $i$.

Case 2: $u$ is the parent of $v$ and they are not on the same heavy path. Using $u_M$ and $v_M$ as before and with the same logic as before but with reversed roles, $b_{v_M} = \ell(u)$. Since $\ell(v) \geq b_{v_M} + 1 = \ell(u) + 1$ because we index depth by 1, and since $\ell(v) = i-1$, we know $i-2 \geq \ell(u)$. This contradicts that $u$ is in $T^i$, and thus this case is impossible. Note that this also shows that $C$ cannot contain a vertex in an ancestor $u_M$ of $v_M$ in $T_M$, because by connectivity, this would imply that there is some $u$ that is the parent of the root of $T_{v_M}$. A similar argument will hold.

Case 3: $u$ and $v$ are on the same heavy path corresponding to meta vertex $u_M$ whose binarized path $T_{u_M}$ has root $r_{u_M}$. Let $P\subseteq P_{u_M}$ be the connected subpath of this heavy path that contains $u$ if we remove all vertices of level $i-1$ or lower. Obviously, $P= C \cap P_{u_M} \subseteq C$. Assume for contradiction that two vertices $p,p'\in P$ have level $i$, so $\ell(p)=\ell(p')=i$.  Let $a = lca_M(p,p')$ be the least common ancestor of $p$ and $p'$ in $T_{u_M}$. Because $a$ is the least common ancestor, one of its children must contain $p$ and the other $p'$ in its subtree. Without loss of generality, assume $p$ is a descendant of the left child and $p'$ is a descendant of the right child.

Let $w$ and $w'$ respectively be the (possibly internal) vertices of $T_{u_M}$ that pass their depth, specifically the lowest depth of all such vertices, to $p$ and $p'$. Thus if $d_{u_M}$ is the depth function in $T_{u_M}$ indexed by 1 and $b_{u_M}$ is the value broadcasted to vertices in $T_{u_M}$ in step 3, then $i=\ell(p) = d_{u_M}(w) + b_{u_M}$ and $i=\ell(p') = d_{u_M}(w') + b_{u_M}$. Since $\ell(p) = \ell(p')$, this implies $d_{u_M}(w) = d_{u_M}(w')$. Additionally, $w$ and $w'$ respectively must be ancestors of $p$ and $p'$ in order to pass their depths to $p$ and $p'$, so they are, respectively, on the paths from $p$ and $p'$ to $r_{u_M}$. Notice that these paths necessarily merge at $a$ and are the same from $a$ to $r_{u_M}$. Since $w$ and $w'$ only pass their depth to exactly one leaf of $T_{u_M}$ each, they must be distinct. Therefore, they cannot be at depth $d_{u_M}(a)$ or lower, else they would be the same vertex on the path from $a$ to $r_{u_M}$ since these paths have exactly one vertex at each depth. Thus, $w$ and $w'$ are strict descendants of $a$, so $d_{u_M}(a) < d_{u_M}(w) = i - b_{u_M}$.

Let $\bar{p}$ be the leftmost leaf descendant of the right child of $a$, where $\bar{p}$ may or may not be equal to $p'$. Then $\bar{p}$ must have been passed the depth $d_{u_M}(a)$, and thus its label is at most $\ell(\bar{p}) \leq d_{u_M}(a) + b_{u_M}$. Then since $d_{u_M}(a) < i - b_{u_M}$, $\ell(\bar{p}) < i - b_{u_M} + b_{u_M} = i$.  
%, also implying that $\bar{p}\neq p,p'$ since their levels are both $i$.
Additionally, note that by the structure of $T_{u_M}$, $\bar{p}$ is located between $p$ and $p'$ in the leaf set, thus it must come between them in the pre-order traversal of $T_{u_M}$. Since $T_{u_M}$ is the binarized path of $P_{u_M}$, this also implies $\bar{p}$ comes between $p$ and $p'$ in $P_{u_M}$, and by extension $P$. Note, however, that $P\subseteq C\subseteq T^i$, and thus its vertices must all have level $i$ or greater. This contradicts that $\ell(\bar{p}) < i$.

Thus far in case 3, we have shown that at most one vertex in $P = C\cap P_{u_M}$ can be at level $i$. We will now show that there is one vertex in $P$ at level $i$. Let $w$ be the right or only child of the vertex that passed its depth to $v$, thus $v$ is the leftmost descendant leaf of $w$. Then $i-1=\ell(v) = d_{u_M}(w) - 1 + b_{u_M}$ so $d_{u_M}(w) = i - b_{u_M}$. Let $p$ be the leftmost descendant of the right child of $w$ and let $a = lcm_{u_M}(v,p)$. Since the left child is just one deeper than $w$, $\ell(p) = d_{u_M}(w) + 1 + b_{u_M} = i + 1$. We now consider a vertex $p'$ between $v$ and $p$ on the heavy path $P_{u_M}$. By Observation~\ref{obs:ancestors}, since $v,p',p$ appear in this order on $P_{u_M}$, $a_{p} = lca_{u_M}(v,p)$ is an ancestor of (or the same as) $a_{p'} = lca_{u_M}(v,p')$. Additionally, since $w$ is an ancestor of both $v$ and $p$, we get the two facts: (1) $w$ is an ancestor of $a_{p'}$ and so $v$ is the leftmost descendant leaf of $a_{p'}$ and (2) the depth of $a_p$ is bounded by the depth of $w$, so $d_{u_M}(a_p) \leq d_{u_M}(w) = i - b_{u_M}$, and since $a_{p'}$ is a descendant of $a_p$ or $a_{p'} = a_p$, $d_{u_M}(a_{p'}) \geq d_{u_M}(a_p) = i  - b_{u_M}$. Since $a_{p'}$ is the lowest common ancestor of $v$ and $p'$, each of its children's subtrees contain exactly one of $v$ or $p'$. Since $v$ is the leftmost descendant leaf, $p'$ must be a descendant of the right child of $a_{p'}$. Therefore, since the vertex $w'$ that passes its depth to $p'$ is the first vertex on the path from $p'$ to $r_{u_M}$ after traversing an edge from a right child, $w'$ must be lower in $T_{u_M}$ than $a_{p'}$. Thus $d_{u_M}(w') \geq d_{u_M}(a_{p'}) \geq i  - b_{u_M}$. Thus the label of $p'$ is $\ell(p') \geq i  - b_{u_M} + b_{u_M} = i $. Therefore, every vertex on the path between $v$ and $p$ is in $T^{i}$. This includes the vertex directly adjacent to $v$ between $v$ and $p$. If this vertex is $u$, we are done.

If this vertex is not $u$, that means $u$ was on the other side of $v$ on the heavy path. Then instead we can let $p$ instead be the leftmost descendant of the right child of the parent of $w$'s other child. The same argument holds, but with reversed orientation.

Finally, all that needs to be shown is that for every vertex $c\in C\setminus P$, $\ell(c) > i$. For any such $c$, let $c^*$ be its lowest ancestor in $P_{u_M}$. Since $\ell(c^*) \geq i$, we can make the same argument as Case 1 to show that $c$ must have label $i+1$ or larger.




%Let $v\in N(C)$ be the vertex at level $i-1$, and let $u\in T_M$ be the meta vertex containing the heavy path with $v$. We start by considering the case where $v$ does not receive a new value from step 2 in this process. Let $d_u$ be the depth function in $T_u$, and let $b_u$ be the broadcasted value for $T_u$. Then $v$'s label is $\ell(v) = d_u(v) + b_u$. Let $v'$ be the vertex immediately before $v$ in the pre-order traversal of $P_u$. Notice it cannot be at level $i-1$, since it would be in the same connected component at level $i-2$ and we know every such component contains only one vertex at level $i-1$.

%Since $v'$ is earlier than $v$ in the traversal, its depth is at most as large as $v$'s depth, so $v'$'s label is at most $\ell(v') \leq d_u(v) + b_u$. Since it doesn't have the same label, $\ell(v)' < d_u(v) + b_u = \ell(v)$. The same argument holds for $v''$ unless its depth is $d_u(v'') = d_u(v)$. Then $\ell(v'') < \ell(v)$ or $\ell(v'') = \ell(v)+1$.


%Now consider the connected components in $T\setminus\{v:\ell(v)<i\}$. We must show that each such component has only one vertex labeled $i$. This is equivalent to saying that for every vertex of level $i-1$, then for every adjacent connected compon


%Consider some $w\in C$, and let $v_M$ and $w_M$ be the meta vertices in $T_M$ that contain $v$ and $w$ respectively in their heavy paths. Additionally, let $v'_M$ and $w'_M$ be the vertices in $T_M'$ that passed their labels to $v$ and $w$ respectively that $v$ and $w$ actually kept. 
%Since we know that every $w\in C\subseteq T\setminus\{v:\ell(v) < i\}$ has label at least $i$, we know that $w$ has  
%TODO
\end{proof}

Next, by showing how it can be implemented in AMPC, we get our following lemma.

\begin{lemma}\label{lem:labelverts}
Given a rooted and oriented meta tree $T_M$ of a tree $T$ with binarized paths whose internal nodes $u$ have access to their associated data $d_u$, a generalized low depth tree decomposition of height $O(\log^2n)$ can be found in $O(1/\epsilon)$ rounds, $O(n^\epsilon)$ local memory, and $O(n\log n)$ total space.
\end{lemma}

\begin{proof}
Correctness has already been shown by Lemma~\ref{lem:decompcorrectness}. All that's left to show is the implementation in AMPC. First, consider each vertex $u\in T_v$ for each meta vertex $v\in T_M$. Since $T_v$ is a complete binary tree with up to $n$ leaves, the max depth by Observation~\ref{obs:binarytree} is $O(\log n)$. Thus, since vertices know their parents, $u$ can adaptively query its path to the root $r_v$ and count the length (plus one since we index by one) with $O(\log n)$ local space for each vertex. This can be done in one round within the local space limitations with $O(n\log n)$ total space. This completes the first step.

The second step is quite simple. Each internal vertex $u\in T_v$ of meta vertex $v\in T_M$ has direct access to its data $d_u$. It simply sends its depth in $T_v$ to $d_u$ in one round. Then, each leaf retains the minimum value sent. This might take up to $O(1/\epsilon)$ rounds to find in parallel for each such leaf. Since there are at most $O(n)$ leaves in binarized paths and each will get at most $O(\log n)$ values (i.e., the max depth of a binarized path), then the total space is at most $O(n\log n)$. Note we did not violate the local space.

Next, consider some $v\in T_M$ with heavy path $P_v$. Since we have the pre-order numbering, we can directly access the first vertex $r$ in the pre-order traversal of $P_v$. Then, simply access $r$'s parent $p$ in the original tree $T$. Since $p$ knows which meta vertex $u$ it is in, we can find $u$ immediately. Now, we need to broadcast $u$'s depth. By Obesrvation~\ref{obs:lightheavy}, the number of heavy paths between a vertex and the root in the original tree $T$ is bounded by $O(\log n)$. Since the heavy paths correspond directly to meta vertices in $T_M$, the path between the vertex and the root in $T_M$ is bounded in length by $O(\log n)$. Then by the same argument as for step 1, $u$ can find its depth in $T_M$ in one round with $O(n^\epsilon)$ local space and $O(n\log n)$ total space. To broadcast the depth, $u$ can send its depth to $v$. In $O(1/\epsilon)$ rounds, $v$ can distribute it to the leaves of $T_v$ in the space constraints.

Step four is again quite simple, since each $u\in T_v$ for $v\in T_M$ has access to the broadcasted value. In one round, each $u$ adds the broadcasted value to its depth. This concludes the proof.
\end{proof}

Now we can finally prove the main lemma of this section

\begin{proof}[Proof of Lemma~\ref{lem:treedecomp}]
By combining Lemmas~\ref{lem:orient},~\ref{lem:heavylight},~\ref{lem:expandverts}, and~\ref{lem:labelverts}, we have our result.
\end{proof}

